Measurement of differential production cross-sections for a $Z$ boson in association with $b$-jets in 7 TeV proton-proton collisions with the ATLAS detector

Measurements of differential production cross-sections of a $Z$ boson in association with $b$-jets in $pp$ collisions at $\sqrt{s}=7$ TeV are reported. The data analysed correspond to an integrated luminosity of 4.6 fb$^{-1}$ recorded with the ATLAS detector at the Large Hadron Collider. Particle-level cross-sections are determined for events with a $Z$ boson decaying into an electron or muon pair, and containing $b$-jets. For events with at least one $b$-jet, the cross-section is presented as a function of the $Z$ boson transverse momentum and rapidity, together with the inclusive $b$-jet cross-section as a function of $b$-jet transverse momentum, rapidity and angular separations between the $b$-jet and the $Z$ boson. For events with at least two $b$-jets, the cross-section is determined as a function of the invariant mass and angular separation of the two highest transverse momentum $b$-jets, and as a function of the $Z$ boson transverse momentum and rapidity. Results are compared to leading-order and next-to-leading-order perturbative QCD calculations.

==> HepData.tex <==
\section{Auxiliary Tables}

\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.78}
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/NPcorr_zb.tex}
  \end{center}
  \caption{Theoretical corrections for the \onetag\ selection. Multiplicative correction factors applied to parton-level theory predictions from MCFM to account for the
softening of the jet spectra due to fragmentation and hadronisation and to the enhancement of the cross-section due to multi-parton interactions (MPI).  A constant QED multiplicative factor, correcting the born lepton definition in MCFM to the dressed definition used in the analysis, is included. The various sources of uncertainties (MC sample size, differences between \pythia\ and \sherpa\ in the modelling of NP-QCD effects, QED final state radiation (FSR) correction and uncertainties on the modelling of the double parton interaction from a comparison to data) are listed separately, along with their quadratic sum.\label{tab:np_zb}}
\end{table}
\normalsize
\newpage


\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.78}
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/NPcorr_zbb.tex}
  \end{center}
  \caption{Theoretical corrections for the \twotag\ selection. Multiplicative correction factors applied to parton-level theory predictions from MCFM to account for the softening of the jet spectra due to fragmentation and hadronisation and to the enhancement of the cross-section due to multi-parton interactions (MPI).  A constant QED multiplicative factor, correcting the born lepton definition in MCFM to the dressed definition used in the analysis, is included. The various sources of uncertainties (MC sample size, differences between \pythia\ and \sherpa\ in the modelling of NP-QCD effects, QED final state radiation (FSR) correction and uncertainties on the modelling of the double parton interaction from a comparison to data) are listed separately, along with their quadratic sum.\label{tab:np_zbb}}
\end{table}
\normalsize
\newpage

\begin{table}[htdp]
\begin{center}
    \renewcommand{\arraystretch}{0.85}
  \setlength{\tabcolsep}{7.0pt}\tiny
  \input{tables/hepdata/SystematicsTable_inc.tex}
  \caption{Systematic uncertainties (in \%) for the cross-section and inclusive $b$-jet cross-sections measured using the \onetag\ selection.
   \label{t:ZbinclSyst}}
\end{center}
\end{table}
\normalsize
\newpage



\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_tobeincl1.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \onetag\ measurement in $b$-jet \pt.\label{tab:systZb1}}
\end{table}                                                                                                              
\normalsize
\newpage
\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_tobeincl2.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \onetag\ measurement in $b$-jet ${|y|}$.\label{tab:systZb2}}
\end{table}                                                                                
\normalsize
\newpage
\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_tobeincl3.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \onetag\ measurement in $y_{boost}$.\label{tab:systZb3}}
\end{table}                                                                                                              
\normalsize
\newpage
\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_tobeincl4.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \onetag\ measurement in ${|\Delta y(Z,b-jet)|}$.\label{tab:systZb4}}
\end{table}                                                                                
\normalsize
\newpage
\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_tobeincl5.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \onetag\ measurement in ${|\Delta \phi(Z,b-jet)|}$.\label{tab:systZb5}}
\end{table}                                                                                                               
\normalsize
\newpage

\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_tobeincl6.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \onetag\ measurement in ${|\Delta R(Z,b-jet)|}$.\label{tab:systZb6}}
\end{table}                                                                                                               
\normalsize
\newpage
\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_tobeincl7.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \onetag\ measurement in $Z$ boson ${p_T}$.\label{tab:systZb7}}
\end{table}
\normalsize
\newpage
\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_tobeincl8.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \onetag\ measurement in $Z$ boson ${|y|}$.\label{tab:systZb8}}
\end{table}
\normalsize
\newpage

\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.78} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystematicsTable_inc_zbb.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the cross-section measured using the \twotag\ selection.\label{tab:systZbb0}}
\end{table}
\normalsize
\newpage

\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.78} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_zbbdiff1.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \twotag\ measurement in $\Delta R(b,b)$.\label{tab:systZbb1}}
\end{table}
\normalsize
\newpage

\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.78} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_zbbdiff2.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \twotag\ measurement in $m(b,b)$.\label{tab:systZbb2}}
\end{table}
\normalsize
\newpage

\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.78} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_zbbdiff3.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \twotag\ measurement in Z boson \pt.\label{tab:systZbb3}}
\end{table}
\normalsize
\newpage

\begin{table}[htdp]
  \begin{center}
    \renewcommand{\arraystretch}{0.78} 
    \setlength{\tabcolsep}{2.5pt}\tiny
    \input{tables/hepdata/SystTable_zbbdiff4.tex}
  \end{center}
  \caption{Systematic uncertainties  (in \%) for the differential \twotag\ measurement in Z boson $|y|$.\label{tab:systZbb4}}
\end{table}
\normalsize

